PEEL the Layers and Find Yourself: Revisiting Inference-time Data Leakage for Residual Neural Networks

This paper explores inference-time data leakage risks of deep neural networks (NNs), where a curious and honest model service provider is interested in retrieving users' private data inputs solely based on the model inference results. Particularly, we revisit residual NNs due to their popularity in computer vision and our hypothesis that residual blocks are a primary cause of data leakage owing to the use of skip connections. By formulating inference-time data leakage as a constrained optimization problem, we propose a novel backward feature inversion method, \textbf{PEEL}, which can effectively recover block-wise input features from the intermediate output of residual NNs. The surprising results in high-quality input data recovery can be explained by the intuition that the output from these residual blocks can be considered as a noisy version of the input and thus the output retains sufficient information for input recovery. We demonstrate the effectiveness of our layer-by-layer feature inversion method on facial image datasets and pre-trained classifiers. Our results show that PEEL outperforms the state-of-the-art recovery methods by an order of magnitude when evaluated by mean squared error (MSE). The code is available at \href{https://github.com/Huzaifa-Arif/PEEL}{https://github.com/Huzaifa-Arif/PEEL}

==> Styles/sec/6_Previous_comments.tex <==
\newpage
\clearpage

\section*{Previous Comments}

The section \textbf{"Previous Comments"} Includes the comment from the previous version. We have copied the comments from the reviews directly without edit. The next section \textbf{"Queries Addressed"} has the answers to the comments that are addressed in our current version.
\begin{itemize}
\item \textbf{Review 1 }
Summary:
This paper investigates the risks of data leakage during inference in deep neural networks, particularly focusing on residual neural networks (ResNets). The study highlights inference-time data leakage, where a model service provider attempts to recover users’ private input data based solely on the model’s inference results. The paper introduces a novel backward feature inversion method called PEEL, which effectively bypasses the computation of ReLU and employs a Laplacian multiplier to mitigate the impact of the non-linear ReLU function in the optimisation process. This approach transforms the problem into an optimisation problem with inequality constraints. By progressively recovering the intermediate outputs of ResNet layers, PEEL can effectively reconstruct input features from these intermediate outputs. Experimental results demonstrate that PEEL achieves an order of magnitude improvement in mean squared error (MSE) compared to existing state-of-the-art recovery methods.

Soundness: 4: excellent
Presentation: 4: excellent
Contribution: 3: good
Strengths:
The paper offers a new perspective on various inverse inference issues related to models and model security problems. Additionally, the proposed method is simple and highly effective for residual networks, which is highly valuable. The logic and reasoning behind each design point are clearly explained and easy to understand.

Weaknesses:
The proposed method has significant limitations, as it seems to be effective only for inverse inference in residual networks, making it difficult to generalize to other models. Additionally, the number of experiments conducted in the critical experimental section is insufficient, lacking a certain degree of persuasiveness.

Questions:
Firstly, why do the images recovered using PEEL generally appear darker than the original images in the paper? What causes this common pattern?

In Figure 6 of the paper, the examples for the Generative based method seem to indicate that the model was not fully trained, as it did not converge well. Can you provide some evidence to show that the model has been properly trained?

The experiments could include one or two additional comparison results with other inversion models to further demonstrate the effectiveness of the method.

Can you provide a preliminary analysis and explanation of why the lack of skip connections or residual propagation causes the method to fail?

Limitations:
The authors demonstrate through experiments in the paper that this method is limited to input inversion for residual networks.

Flag For Ethics Review: No ethics review needed.
Rating: 6: Weak Accept: Technically solid, moderate-to-high impact paper, with no major concerns with respect to evaluation, resources, reproducibility, ethical considerations.
Confidence: 4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.
Code Of Conduct: Yes

\item \textbf{Review # 2 }

Summary:
The authors have proposed an inference-time data leakage black-box attack, where a service provider (model owner) is honest but curious and tries to reconstruct the input image from a network's output (logits). Authors have devised a method termed PEEL, which sequentially, in a recursive manner, recovers the input image from each residual block in a network with the residual connection.

Soundness: 2: fair
Presentation: 3: good
Contribution: 2: fair
Strengths:
The proposed attack is a black-box attack, without access to intermediate layers' output.
The evaluation is thorough and the authors have shown results on vision transformers too.
The success of the attack does not depend on the weights learned during the training, and works even for the randomly initialized networks.
Weaknesses:
This work lacks novel insights, in terms of the success of their attack methods. Authors have shown that success does not depend on the actual weights of the network. This raises the question, of what it depends on (apart from the residual architecture)

 Does it depend on the non-linearity in the network? If yes, then it must be evaluated on the wider version of ResNet18 networks, since increasing the width effectively linearized the model [1,2].

 Further, how does the effectiveness of PEEL depend on the distribution of nonlinearity (ReLUs)? For instance, a baseline ResNet18 network and their HybReNets counterparts [2], HRN-5x5x3x and HRN-2x5x3x networks, have distinct ReLUs' distributions. A thorough study of the impact of various non-standard ReLU distributions could have provided valuable insights into the network design strategies to prevent inference-time data leakage.

 Moreover, this investigation is required to verify the authors' hypothesis that whether "Residual blocks are the primary cause of data leakage" or the nonlinearities in the network also play a crucial role in the success of PEEL.

Also, the practical utility of this attack and the threat model is not clear. In particular, Why do service providers try to reconstruct the users' data? An honest-but-curious client makes sense, however, the model owner would be risking their own business, if they do perform any data-leakage attack.

[1] Lee et al., ide neural networks of any depth evolve as linear models under gradient descent, NeurIPS 2019.

[2] Jha et al., DeepReShape: Redesigning Neural Networks for Efficient Private Inference, TMLR 2024.

Questions:
Given the fact that non-linearities make feature-based inversion attacks difficult, what if we remove the non-linearities from the network? For example, if we remove the stage-wise nonlinearity (stage to stage, one at a time) then would it impact the success of the feature-based inversion attacks (Similar to ReLU Culling used in [4])? Or, if we drop the ReLUs from the alternate layers in ResNet18, which is shown to be beneficial without impacting the network's performance [3,4] (ReLU-Thinning used in [4])

see other points in weaknesses.

[3] Zhao et al. Rethinking ReLU to Train Better CNNs, ICPR 2018.

[4] Jha et al., DeepReDuce: ReLU Reduction for Fast Private Inference, ICML 2021.

Limitations:
Addresses in the paper.

Flag For Ethics Review: No ethics review needed.
Rating: 4: Borderline reject: Technically solid paper where reasons to reject, e.g., limited evaluation, outweigh reasons to accept, e.g., good evaluation. Please use sparingly.
Confidence: 3: You are fairly confident in your assessment. It is possible that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work. Math/other details were not carefully checked.
Code Of Conduct: Yes

\item \textbf{Reviewer # 3}
Summary:
This paper examines the risk of inference-time data leakage in deep neural networks, focusing on resnets. It introduces a novel backward feature inversion method, PEEL, which effectively recovers block-wise input features from the intermediate outputs of resnets. The emprical methods suggest the method can outperform other peer generative model based methods.

Soundness: 2: fair
Presentation: 3: good
Contribution: 3: good
Strengths:
the paper studies a fairly new setting and demonstrate interesting results in comparison to generative based method.
the method is fairly straightforward and paper is fairly easy to follow.
the results appear quite impressive (more in questions).
Weaknesses:
The setting of HbC is a bit un-intuitive, in particular, if the party-B is holding the model as a service, and if they are curious about hte input, why they cannot directly examine the input to check what the input is, but have to use the predicted results to infer the input? The authors have cited several works to support the setting of HbC, however, it appears these works are typically discuss the setting in distributed setting or federated learning setting. However, the authors seem to only discuss this and test this empirically in local model setting.
The empirical discussion is a bit thin, the results over CelebA and chestXray are quite impressive, it's a bit unclear why the authors do not use more standard setting and models typically in computer vision (e.g., cifar and ImageNet)
Questions:
the empirical part is a bit unclear, for example, there are many details about the model in CelebA, but not so much details about the dataset and models in the ChestXray setting.
More relevant results in more standard setting can make the work more convincing. The impressive results might be due to the simplified setting, for example, there are only 2 classes with 30 samples each? (line 262)
Limitations:
the authors have a clearly stated limitation discussion.

Flag For Ethics Review: No ethics review needed.
Rating: 4: Borderline reject: Technically solid paper where reasons to reject, e.g., limited evaluation, outweigh reasons to accept, e.g., good evaluation. Please use sparingly.
Confidence: 3: You are fairly confident in your assessment. It is possible that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work. Math/other details were not carefully checked.
Code Of Conduct: Yes
\end{itemize}

\section*{Queries adddressed}


\begin{itemize} 

\item \textbf{Reviewer 1} requested evidence that the generative method used as a baseline is indeed converging. In response, we have provided evidence in Appendix (Section J), demonstrating that the target model was fully trained and that distributional recovery is converging. Additionally, we conducted new experiments incorporating another baseline, Embedding Inversion, alongside KEDMI-LOMMAA, which are now reflected in Figure 6 and Tables 2 and 3 of the main paper. The reviewer also asked why PEEL images appear darker when pretrained weights are used. The darkness is due to the large pretrained weights that PEEL has to handle. As discussed in the experimental section, "Since PEEL is a numerical solver, the quality of the reconstruction decreases when large pretrained weights are used for recovery."

\item \textbf{Reviewer 2} raised concerns about the impact of non-linearity within the architecture. To address this, we performed experiments on architectures without non-linearity, such as those lacking PReLU activation. The results, found in Figure 15 and Section D of the Ablation Study, show that PEEL’s effectiveness in data recovery is primarily dependent on the presence of residual connections rather than the non-linearity of the activation function. Additionally, in response to the reviewer’s request for clarification on the "distribution of nonlinearities," we conducted further experiments using Hybrid ResNets with varying distributions of non-linearities in addition to the base ResNet-18 model. These experiments, which examine the effect of different ResNet widths on data leakage, are addressed in Section E of the Ablation Study. Furthermore, we discussed the HbC (Honest but Curious) setting in Section A of the Introduction, highlighting security risks where model providers, restricted from viewing input directly, might still recover input data from intermediate representations during inference.

\item \textbf{Reviewer 3} inquired about the relevance of the HbC setting, which is discussed in detail in Section A of the Introduction. The reviewer also requested additional experiments involving PEEL on samples from the standard ImageNet and CIFAR datasets, which are now included in Section B of the Ablation Study. Moreover, the reviewer requested similar experiments on the Chest X-ray dataset, akin to those conducted on CelebA. We addressed this by performing comprehensive evaluations using ResNet architectures of varying depths and presenting results for the Chest X-ray dataset under different configurations, such as with and without pretraining. These results are detailed in Section A (Figures 12 and 13) of the Ablation Study and include the use of pooling layers, analogous to the evaluations performed on CelebA in the original paper.


\end{itemize}





